A Floer homology for exact contact embeddings

In this paper we construct the Floer homology for an action functional which was introduced by Rabinowitz and prove a vanishing theorem. As an application, we show that there are no displaceable exact contact embeddings of the unit cotangent bundle of a sphere of dimension greater than three into a convex exact symplectic manifold with vanishing first Chern class. This generalizes Gromov's result that there are no exact Lagrangian embeddings of a sphere into a complex vector space.

==> f1 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 0 100 0 20 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3000 2250 4500 2250
2 1 2 1 0 0 100 0 20 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 4500 2250 6225 2250
2 1 0 1 0 0 100 0 20 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 4425 2250 4425 4125
2 1 0 1 0 0 100 0 20 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 4425 4125 5175 4125
2 1 0 1 0 0 100 0 20 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5175 4125 5175 4875
2 1 0 1 0 0 100 0 20 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5175 4875 6300 4875
2 1 2 1 0 7 100 0 -1 3.000 0 0 -1 1 0 3
	0 0 1.00 60.00 120.00
	 5175 4125 6075 4125 6150 4125
2 1 2 1 0 7 100 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3600 4125 4425 4125
2 1 2 1 0 7 100 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 4350 4875 5250 4875
2 2 0 1 0 0 100 0 20 3.000 0 0 -1 0 0 5
	 6300 4800 6450 4800 6450 4950 6300 4950 6300 4800
2 2 0 1 0 0 100 0 20 0.000 0 0 -1 0 0 5
	 2850 2175 3000 2175 3000 2325 2850 2325 2850 2175
4 0 0 100 0 0 12 0.0000 2 195 2085 4725 4050 $\\dot{y_1}=-\\nabla h(y_1)$\001
4 0 0 100 0 0 12 0.0000 6 195 2055 3000 3150 $\\dot{x_1}=-\\nabla f(x_1)$\001
4 0 0 100 0 0 12 0.0000 0 135 1965 4275 5475 A flow line with cascades\001

